Transcoding Billions of Unicode Characters per Second with SIMD Instructions

In software, text is often represented using Unicode formats (UTF-8 and UTF-16). We frequently have to convert text from one format to the other, a process called transcoding. Popular transcoding functions are slower than state-of-the-art disks and networks. These transcoding functions make little use of the single-instruction-multiple-data (SIMD) instructions available on commodity processors. By designing transcoding algorithms for SIMD instructions, we multiply the speed of transcoding on current systems (x64 and ARM). To ensure reproducibility, we make our software freely available as an open source library.

==> garbage.tex <==



State machines are wonderful tools
\url{https://nullprogram.com/blog/2020/12/31/}

encoding\_rs:
a Web-Compatible Character Encoding Library in Rust
\url{https://hsivonen.fi/encoding_rs/}

Even faster UTF-8 character counting \url{http://www.daemonology.net/blog/2008-06-05-faster-utf8-strlen.html}

The fastest way to html encode string to Utf8 string
https://github.com/dotnet/runtime/issues/35004

https://github.com/hsivonen/kewb
kewb
Bob Steagall’s SSE2-accelerated converter presented at CppCon2018 

TextEncoder.encodeInto and TextDecoder.decode APIs.




UTF-8 processing using SIMD (SSE4) \url{https://woboq.com/blog/utf-8-processing-using-simd.html}
 


UTF16 - https://tools.ietf.org/html/rfc2781
UTF8 - https://tools.ietf.org/html/rfc3629

V8 utf-8 decoder: https://github.com/v8/v8/blob/master/src/third_party/utf8-decoder/utf8-decoder.h

C# utf8 encoder https://github.com/dotnet/runtime/blob/master/src/libraries/System.Private.CoreLib/src/System/Text/UTF8Encoding.cs


JVM, .Net, Chrome, Mozilla, Microsoft libc, BSD, GNU, Rust ... all use different UTF-8 decoders.

branchless utf8 https://github.com/skeeto/branchless-utf8

\section{Software}

\begin{itemize}
\item \url{https://github.com/stgatilov/utf8lut} and 
        \item encoding\_rs in rust is probably the state of the art? It does use SIMD but only(?) for the ASCII ranges. See \url{https://github.com/hsivonen/encoding_rs/blob/master/src/simd_funcs.rs}
    \item \url{https://github.com/KWillets/fastdecode-utf-8} (probably unfinished)
    \item iconv?
    \item ICU
    \item https://github.com/hsivonen/kewb
    
    

\end{itemize}

